NuGrid stellar data set I. Stellar yields from H to Bi for stars with metallicities Z = 0.02 and Z = 0.01

We provide a set of stellar evolution and nucleosynthesis calculations that applies established physics assumptions simultaneously to low- and intermediate-mass and massive star models. Our goal is to provide an internally consistent and comprehensive nuclear production and yield data base for applications in areas such as pre-solar grain studies. Our non-rotating models assume convective boundary mixing where it has been adopted before. We include 8 (12) initial masses for $Z = 0.01$ ($0.02$). Models are followed either until the end of the asymptotic giant branch phase or the end of Si burning, complemented by a simple analytic core-collapse supernova models with two options for fallback and shock velocities. The explosions show which pre-supernova yields will most strongly be effected by the explosive nucleosynthesis. We discuss how these two explosion parameters impacts the light elements and the $s$ and $p$ process. For low- and intermediate-mass models our stellar yields from H to Bi include the effect of convective boundary mixing at the He-intershell boundaries and the stellar evolution feedback of the mixing process that produces the $^{13}$C pocket. All post-processing nucleosynthesis calculations use the same nuclear reaction rate network and nuclear physics input. We provide a discussion of the nuclear production across the entire mass range organized by element group. All our stellar nucleosynthesis profile and time evolution output is available electronically, and tools to explore the data on the NuGrid VOspace hosted by the Canadian Astronomical Data Centre are introduced.

==> astronat/doc/Makefile <==

# $Id: Makefile,v 1.4 1999/09/01 03:33:59 jbaker Exp $

MAKEINFO = makeinfo
TEXI2DVI = texi2dvi
TEXI2HTML = texi2html
DVIPS = dvips

TEXI2HTML_FLAGS =  -verbose -split_chapter

HTMLDIR = ./html
TEXDIR = ./tex

SRC = astronat
TEXI = $(SRC).texi


all : info text html # ps

info : $(TEXI)
	$(MAKEINFO) --verbose $(TEXI)

text : $(TEXI)
	$(MAKEINFO) --no-headers $(TEXI) > $(SRC).txt

html : $(TEXI)
	if [ ! -d $(HTMLDIR) ]; then mkdir $(HTMLDIR); fi
	cd $(HTMLDIR); $(TEXI2HTML) $(TEXI2HTML_FLAGS) ../$(TEXI); \
	if [ -f index.html ]; then $(RM) index.html; fi; \
	ln -s astronat_toc.html index.html

ps : $(TEXI)
	if [ ! -d $(TEXDIR) ]; then mkdir $(TEXDIR); fi
	cd $(TEXDIR); $(TEXI2DVI) ../$(TEXI); $(DVIPS) -o $(SRC).ps $(SRC); \
	mv $(SRC).ps $(SRC).dvi ..

clean :
	-$(RM) $(SRC).info $(SRC).txt $(SRC).dvi $(SRC).ps
	-$(RM) -r $(HTMLDIR) $(TEXDIR)

